Batch-Dynamic Coreness and Applications with Logarithmic Work via Balanced Pressures

We give a parallel algorithm that maintains a one-sided $(2+\varepsilon)$-approximation of all core numbers under batches of edge insertions and deletions. For fixed $\varepsilon>0$, the expected amortized work is $O(\log n)$ per edge update, and each batch has deterministic polylogarithmic depth. This improves on the previously known $(4+\varepsilon)$-approximation and $O(\log^2 n)$ amortized work bounds. This approximation factor approaches the factor-two limit for polylogarithmic update and query time under the OMv conjecture. Our algorithm is based on assigning each vertex a "pressure" and splits each edge's unit load smoothly between its endpoints according to their pressures. After each batch of updates, our dynamic algorithm adjusts the pressures of vertices in parallel to restore balance between the pressures and loads. We show that by maintaining balanced pressures we can obtain good approximations of core numbers. Our construction also gives a $(1+\varepsilon)$-approximation of the densest-subgraph value with logarithmic expected amortized work and supports batch-dynamic maximal matching, clique counting, forest decomposition, and coloring in low-arboricity graphs with improved or matching work bounds. We give a practical implementation of our batch-dynamic coreness algorithm and find that it is able to achieve smaller empirical error than the state-of-the-art parallel batch-dynamic implementation, while running faster. On six real-world graphs, it runs $32\times$ faster than that implementation in geometric mean and $4.1\times$ faster than a state-of-the-art heuristic baseline. On three graphs with up to 1.8 billion edges, it is $9.2\times$ faster than the heuristic baseline.

==> sections/worst-case.tex <==
\section{Worst-Case Coreness via Balanced Orientations}\label{app:worst-case}

Our weighted peeling argument also gives a one-sided $(2+\eps)$ coreness
approximation with worst-case batch bounds, using the orientation algorithm
of Ghaffari--Koo~\cite{GK25}. Their algorithm moves units of out-degree
between vertices by reversing edges, using a parallel token-dropping
procedure to process a batch. It maintains an \emph{$H$-balanced orientation}:
writing $d(v)$ for out-degree and $x(v)=\min\{d(v),H\}$, every arc $u\to v$
satisfies $x(u)\le x(v)+1$. The update cost is polynomial in $H$ and
$\log n$. They keep $H$ polylogarithmic by replicating or sampling edges
at different scales. We sharpen the relation between these orientations
and core numbers; their orientation algorithm is unchanged.

\begin{lemma}\label{lem:wc-balanced}
In an $H$-balanced orientation, for every vertex $v$ and $0<\delta\le1$,
\[
 \min\{d(v),H\}\le(1+\delta)k(v)+\frac{2\ln n}{\delta}.
\]
The statement also holds for multigraphs, with degrees counting multiplicity.
\end{lemma}
\begin{proof}
Fix $v$, let $k=k(v)$, and let $S$ be the prefix ending at $v$ in a peeling
order. Each vertex of $S$ has at most $k$ later neighbors. Set
$\lambda=\ln(1+\delta)$ and $w(u)=e^{\lambda x(u)}$.
An arc within $S$ contributes its tail's weight to
$\sum_{u\in S}d(u)w(u)$. By balance, this is at most $e^\lambda$ times
the weight of its earlier endpoint. An arc leaving $S$
contributes that endpoint's weight; an arc entering $S$ contributes zero.
Since $x(u)\le d(u)$, charging to earlier endpoints gives
\[
 \sum_{u\in S}x(u)w(u)
 \le e^\lambda k\sum_{u\in S}w(u).
\]
Put $Z=\sum_{u\in S}w(u)$ and $\pi(u)=w(u)/Z$. Since the entropy of a
distribution on $S$ is at most $\ln|S|$,
\begin{align*}
 \ln Z&=\lambda\sum_{u\in S}\pi(u)x(u)-\sum_{u\in S}\pi(u)\ln\pi(u)\\
 &\le\lambda e^\lambda k+\ln n.
\end{align*}
Since $\lambda x(v)\le\ln Z$, divide by $\lambda$ and use
$\ln(1+\delta)\ge\delta/2$.
\end{proof}

\begin{corollary}\label{cor:wc-coreness}
For every fixed $0<\eps\le1$, a batch-dynamic data structure maintains
\[
                 \frac{k(v)}{2+\eps}\le\widehat{k}(v)\le k(v)
\]
with constant-time estimate queries, $O(b\log^9 n)$ worst-case work and
$O(\log^7 n)$ depth per batch of $b$ updates in the CRCW PRAM model.
After $O(n\log n)$ initialization work, the guarantee holds with high
probability over any fixed polynomial-length update sequence starting
from the empty graph.
\end{corollary}
\begin{proof}
We spell out the adjustment to Ghaffari--Koo's scale reduction
\cite[Section~5]{GK25}. Set $\delta=\eps/64$,
$A=C\log n/\delta$ for a sufficiently large constant $C$, and
$B=\lceil A/\delta\rceil$. Use scales $h_i=(1+\delta)^i$ from $1$ up to
the first scale at least $2n$. At a scale $h=h_i\le B$, replicate every
edge $a=\lceil B/h\rceil$ times; at a scale $h>B$, sample edges independently
with probability $a=B/h$, retaining each sampling decision until deletion.
Write $a_i=a$ for this scale, so $B\le ah\le2B$. Use cap
$H=2a\lceil h\rceil$ for replication and $H=2B$ for sampling; in both
cases $H\ge2ah$ and $H=O(B)$. Write $x_i(v)=\min\{d_i(v),H\}$.

Let $k_i$ be the core numbers in the graph at scale $i$. Replication is
exact; the sampling bounds~\cite[Lemmas~A.1--A.2]{GK25} give, simultaneously
over vertices, scales and batch boundaries, with high probability,
\[
       |k_i(v)-a k(v)|\le\delta a k(v)+A.
\]
Lemma~\ref{lem:wc-balanced} then gives
\[
             x_i(v)\le(1+\delta)^2a k(v)+(2+\delta)A.
\]
If $x_i(v)<ah$, then $d_i(v)=x_i(v)<H-A$, since $A\le\delta ah$.
Ghaffari--Koo's lower bound~\cite[Lemma~3.4]{GK25} applies in this case:
\begin{align*}
 x_i(v)&\ge(1/2-\delta)k_i(v)-A\\
       &\ge(1/2-\delta)(1-\delta)a k(v)-(3/2-\delta)A.
\end{align*}
These inequalities and $A/(ah)\le\delta$ imply the two tests
\begin{equation}\label{eq:wc-tests}
 \begin{aligned}
 x_i(v)<a_i h_i&\ \Longrightarrow\ k(v)\le(2+10\delta)h_i,\\
 x_i(v)\ge a_i h_i&\ \Longrightarrow\ k(v)\ge(1-4\delta)h_i.
 \end{aligned}
\end{equation}

For a non-isolated vertex, choose the first scale $h_i$ passing the first
test. Such a scale exists by the second test and $k(v)<n$. If $i>0$, the
preceding scale fails, so~\eqref{eq:wc-tests} gives
\[
              (1-5\delta)h_i\le k(v)\le(2+10\delta)h_i.
\]
The same bounds hold for $i=0$, since then $h_i=1$ and $k(v)\ge1$.
Report $\widehat{k}(v)=(1-5\delta)h_i$, and zero for isolated vertices.
The approximation follows from
$(2+10\delta)/(1-5\delta)\le2+\eps$.

Finally, all caps are $O(B)$. Summing the geometric replication factors
and the sampled scales gives $O(B)$ edge copies per update for fixed
$\eps$. The orientation primitive~\cite[Theorem~4.1 and Corollary~5.4]{GK25}
therefore uses $O(bB^7\log n)$ work and $O(B^6\log n)$ depth.
Store degrees and estimates in arrays indexed by vertex and scale.
Collect vertices whose out-degrees change, together with the batch endpoints,
and recompute their estimates by scanning the $O(\log n)$ scales.
Sorting these identifiers and performing
the scans adds at most a factor $O(\log n)$ in work and
$O(\log^2 n)$ depth. Since $B=O(\log n)$, this gives the stated bounds
and stores one estimate per vertex. Mixed batches process deletions before
insertions.
\end{proof}


==> tables/breakeven_rows.tex <==
% generated by scripts/paper_breakeven.py
\multirow{3}{*}{\emph{stackoverflow}} & Ins & $1.3\cdot10^{4}$ & $5.6\cdot10^{5}$ & $5.9\cdot10^{6}$ \\
 & Del & $7.8\cdot10^{4}$ & $1.3\cdot10^{6}$ & $>10^{7}$ \\
 & Mix & $6.3\cdot10^{4}$ & $9.3\cdot10^{5}$ & never \\
\midrule
\multirow{3}{*}{\emph{livejournal}} & Ins & $1.3\cdot10^{4}$ & $8.7\cdot10^{5}$ & $8.7\cdot10^{6}$ \\
 & Del & $1.2\cdot10^{5}$ & $1.8\cdot10^{6}$ & $8.4\cdot10^{6}$ \\
 & Mix & $7.7\cdot10^{4}$ & never & never \\
\bottomrule%


==> tables/main_rows.tex <==
% generated by scripts/paper_tables.py
\multirow{3}{*}{\emph{dblp}} & Ins & 10.4 & 1107 & 49.7 & \textbf{11.1} & 15451 & 2.66 & 1.97 & \textbf{1.48} & 1.03 & 4.00 & 3.00 & 2.83 & 1.50 \\
 & Del & 1.79 & 44.8 & 13.1 & \textbf{3.46} & 14788 & \textbf{1.51} & 2.37 & 1.65 & 1.01 & 2.00 & 6.00 & 2.31 & 2.00 \\
 & Mix & 7.85 & 1305 & 68.7 & \textbf{14.2} & 17142 & 1.54 & \textbf{1.31} & 1.38 & 1.01 & 4.00 & 4.00 & 2.97 & 2.00 \\
\midrule
\multirow{3}{*}{\emph{youtube}} & Ins & 20.1 & 849 & 68.9 & \textbf{21.3} & 18990 & 1.71 & 1.43 & \textbf{1.18} & 1.01 & 4.00 & 3.00 & 3.03 & 2.00 \\
 & Del & 16.0 & 69.3 & 29.2 & \textbf{12.0} & 15676 & 1.45 & \textbf{1.25} & 1.30 & 1.01 & 4.00 & 3.00 & 3.03 & 2.00 \\
 & Mix & 25.6 & 600 & 67.9 & \textbf{20.8} & 17259 & 1.58 & 1.33 & \textbf{1.22} & 1.01 & 4.00 & 3.00 & 3.03 & 2.00 \\
\midrule
\multirow{3}{*}{\emph{wiki}} & Ins & 17.2 & 1232 & 61.5 & \textbf{20.6} & 9006 & 1.66 & 1.52 & \textbf{1.09} & 1.01 & 4.17 & 3.00 & 2.42 & 1.52 \\
 & Del & 12.6 & 77.4 & 22.8 & \textbf{8.68} & 11970 & 1.54 & 1.45 & \textbf{1.12} & 1.00 & 4.00 & 4.00 & 2.42 & 1.38 \\
 & Mix & 18.5 & 165 & 39.9 & \textbf{20.7} & 8712 & 1.53 & 1.41 & \textbf{1.15} & 1.01 & 4.00 & 3.00 & 2.42 & 1.45 \\
\midrule
\multirow{3}{*}{\emph{stackoverflow}} & Ins & 69.9 & 839 & 99.2 & \textbf{21.7} & 18729 & 2.54 & 1.97 & \textbf{1.15} & 1.07 & 4.17 & 3.00 & 2.75 & 1.52 \\
 & Del & 65.6 & 284 & 57.0 & \textbf{15.4} & 20033 & 1.73 & 1.49 & \textbf{1.32} & 1.04 & 4.00 & 4.00 & 2.75 & 1.47 \\
 & Mix & 110 & 660 & 116 & \textbf{13.7} & 12863 & 2.50 & 1.94 & \textbf{1.15} & 1.07 & 4.17 & 3.00 & 2.70 & 1.52 \\
\midrule
\multirow{3}{*}{\emph{livejournal}} & Ins & 132 & 1890 & 147 & \textbf{34.0} & 26286 & 2.62 & 1.83 & \textbf{1.23} & 1.07 & 4.17 & 3.00 & 3.11 & 1.53 \\
 & Del & 129 & 427 & 88.4 & \textbf{30.5} & 25249 & 1.60 & \textbf{1.28} & 1.33 & 1.03 & 4.00 & 4.00 & 3.11 & 2.00 \\
 & Mix & 223 & 1369 & 143 & \textbf{18.4} & 18687 & 2.60 & 1.82 & \textbf{1.23} & 1.07 & 4.17 & 3.00 & 3.11 & 1.53 \\
\midrule
\multirow{3}{*}{\emph{orkut}} & Ins & 247 & 2135 & 178 & \textbf{30.3} & 30260 & 3.33 & 2.02 & \textbf{1.24} & 1.21 & 4.17 & 3.00 & 2.30 & 1.52 \\
 & Del & 243 & 987 & 136 & \textbf{30.1} & 30291 & 1.70 & \textbf{1.24} & 1.25 & 1.10 & 4.00 & 4.00 & 2.38 & 1.40 \\
 & Mix & 395 & 1389 & 183 & \textbf{17.8} & 19072 & 3.32 & 2.01 & \textbf{1.24} & 1.20 & 4.17 & 3.00 & 2.30 & 1.52 \\
\midrule
\multirow{3}{*}{\emph{brain}} & Ins & 333 & 1703 & 166 & \textbf{36.4} & -- & 3.49 & 1.86 & \textbf{1.27} & -- & 4.19 & 3.00 & 3.01 & -- \\
 & Del & 302 & -- & 213 & \textbf{39.0} & -- & -- & 1.25 & \textbf{1.24} & -- & -- & 4.00 & 3.01 & -- \\
 & Mix & 441 & -- & 340 & \textbf{15.7} & -- & -- & 1.86 & \textbf{1.27} & -- & -- & 3.00 & 3.01 & -- \\
\midrule
\multirow{3}{*}{\emph{twitter}} & Ins & 1683 & 1874 & 344 & \textbf{59.7} & -- & 3.16 & 2.27 & \textbf{1.25} & -- & 4.20 & 3.00 & 3.02 & -- \\
 & Del & 1686 & -- & 323 & \textbf{30.6} & -- & -- & 1.34 & \textbf{1.32} & -- & -- & 4.00 & 2.55 & -- \\
 & Mix & 2662 & -- & 654 & \textbf{25.4} & -- & -- & 2.26 & \textbf{1.25} & -- & -- & 3.00 & 3.02 & -- \\
\midrule
\multirow{3}{*}{\emph{friendster}} & Ins & 3108 & 3244$^*$ & 269 & \textbf{34.5} & -- & -- & 1.95 & \textbf{1.22} & -- & -- & 3.00 & 3.00 & -- \\
 & Del & 2943 & -- & 203 & \textbf{33.0} & -- & -- & \textbf{1.27} & 1.31 & -- & -- & 4.00 & 2.59 & -- \\
 & Mix & 4884 & -- & 273 & \textbf{23.5} & -- & -- & 1.95 & \textbf{1.22} & -- & -- & 3.00 & 3.00 & -- \\
\bottomrule%


==> tables/moves_rows.tex <==
% generated by scripts/paper_tables.py
\emph{dblp} & 13.0 & 0.41 & 0.90 & 0.18 & 0.18 & 0.25 & 7.32 & 0.24 & 0.43 \\
\emph{youtube} & 3.01 & 0.21 & 1.11 & 0.09 & 0.09 & 0.54 & 1.03 & 0.12 & 0.60 \\
\emph{wiki} & 2.95 & 0.11 & 0.82 & 0.05 & 0.05 & 0.05 & 0.07 & 0.02 & 0.68 \\
\emph{stackoverflow} & 0.97 & 0.15 & 0.30 & 0.10 & 0.09 & 0.17 & 0.32 & 0.08 & 0.19 \\
\emph{livejournal} & 5.85 & 0.30 & 1.23 & 0.26 & 0.18 & 1.00 & 2.13 & 0.11 & 0.27 \\
\emph{orkut} & 3.97 & 0.20 & 0.60 & 0.31 & 0.14 & 0.51 & 0.81 & 0.04 & 0.08 \\
\bottomrule%


==> tables/road_rows.tex <==
% generated by scripts/paper_tables.py
\multirow{3}{*}{\emph{ctr}} & Ins & 58.9 & 25.8 & \textbf{23.4} & 25.7 & 8713 & 1.71 & \textbf{1.60} & 1.78 & 1.01 & 3.00 & 3.00 & 2.67 & 2.00 \\
 & Del & 93.6 & \textbf{46.5} & 46.9 & 55.2 & 9652 & 1.28 & \textbf{1.23} & 1.71 & 1.00 & 3.00 & 3.00 & 2.55 & 2.00 \\
 & Mix & 111 & 43.9 & \textbf{43.7} & 46.2 & 9770 & 1.68 & \textbf{1.57} & 1.74 & 1.01 & 3.00 & 3.00 & 2.60 & 2.00 \\
\midrule
\multirow{3}{*}{\emph{usa}} & Ins & 99.3 & 25.1 & \textbf{22.5} & 25.9 & 7142 & 1.71 & \textbf{1.60} & 1.79 & 1.01 & 3.00 & 3.00 & 2.88 & 2.00 \\
 & Del & 163 & \textbf{48.2} & \textbf{48.2} & 58.8 & 9786 & 1.27 & \textbf{1.23} & 1.75 & 1.01 & 3.00 & 3.00 & 2.58 & 2.00 \\
 & Mix & 193 & 44.0 & \textbf{43.9} & 46.6 & 9775 & 1.69 & \textbf{1.58} & 1.77 & 1.01 & 3.00 & 3.00 & 2.88 & 2.00 \\
\bottomrule%

